Community-aware network sparsification

Network sparsification aims to reduce the number of edges of a network while maintaining its structural properties; such properties include shortest paths, cuts, spectral measures, or network modularity. Sparsification has multiple applications, such as, speeding up graph-mining algorithms, graph visualization, as well as identifying the important network edges. In this paper we consider a novel formulation of the network-sparsification problem. In addition to the network, we also consider as input a set of communities. The goal is to sparsify the network so as to preserve the network structure with respect to the given communities. We introduce two variants of the community-aware sparsification problem, leading to sparsifiers that satisfy different connectedness community properties. From the technical point of view, we prove hardness results and devise effective approximation algorithms. Our experimental results on a large collection of datasets demonstrate the effectiveness of our algorithms.

==> problem.tex <==
\section{Constructing network from sets}\label{sec:problem}

\begin{problem}\label{problem:general}
Given property $\calP$, a graph $G=(V, E)$ and $\ell$ subsets
$S_1,\ldots, S_\ell$ such that 
$S_i\subseteq V$, find $G' = (V, E')$ with 
$E' \subseteq E$ such that
$f_\calP(S_i; G') = 1$ and $|E'|$ is minimized. 
\end{problem}

\note{Talk about G being optional}

%\mpara{:}
When {\calP} is \emph{connectivity} then Angluin \etal~\cite{angluin13connectivity} have studied this problem 
and showed that it is {\NP}-hard, while the number of edges can be approximated 
within a factor of $O(\log \ell)$, where $\ell$ is the number of subsets of $V$ on which the
connectivity property must hold.


==> s2n-abstract.tex <==
While in most graph-mining problems it is assumed 
that the network is given as input, 
there are many interesting applications in which the network structure is not known
and it is useful to reconstruct it. 
This consideration leads to a general class of {\em network-reconstruction problems}, 
in which the input consists of
observations that represent different manifestations of an underlying, yet \emph{unseen}, network structure
and  the goal is to reconstruct this unseen network. 

In this paper, we focus on combinatorial formulations 
of the general network-reconstruction problem. 
In particular, we assume that our input consists of a collection of sets,
which represent subgraphs of the underlying network.
Further, we assume that these sets satisfy a certain \emph{connectedness property}
in the unseen network. 
Our goal is to construct a \emph{sparse} network
that resembles the underlying network and thus guarantees the same connectedness property
for the input sets of nodes.
We consider three such connectedness properties: 
connectivity, density, and star containment.
While connectivity has been addressed by previous work~\cite{angluin13connectivity}, 
we are the first to study the other two properties.
For the properties we consider, 
we establish the complexity of the corresponding problems, 
and we present efficient approximation algorithms.
We experimentally validate our methods on datasets where 
ground-truth networks are available; 
our results show that the networks constructed by our methods
recover individual edges of the ground-truth networks with relatively high accuracy. 


==> s2n-introduction.tex <==
\section{Introduction}
\label{sec:intro}

In most graph-mining problems it is assumed that the network structure is known. 
Classic problems such as
community detection, 
frequent subgraph mining, 
identification of central nodes and edges are
all examples  in which the network structure is part of the input. 



\begin{figure}
\begin{center}
\input{introfigure}	
\caption{\label{figure:intro}Reconstructing a network from a collection of sets.
In this case, in the reconstructed network,
each of the input sets induces a subgraph of density at least~$3/2$, 
where density is defined as the average degree of a node in the subgraph.}
\end{center}
\end{figure}

However, there are many cases in which the network structure is unknown
and only a manifestation of it is available. 
For example,
a large company may have data about past projects, 
including information whether which projects were successful and which not, 
and which employees participated in each project.
It is natural to assume that the team composition of the employees in the different projects
depends on an underlying network
that models the complementarity of skills, 
the synergy between the employees, 
and their capacity to work together.
However, such a network may not be available in our data
and we would like to infer it.
The motivation for inferring the structure of such a hidden network
is that it can be used for creating successful teams for future projects. 
For instance, in the work of Lappas et al.\ on 
\emph{team formation}~\cite{lappas09finding}, 
it is assumed
that the algorithm has access to a network,
which models the collaboration capacity between different individuals. 

\iffalse
In other cases, only partial or uncertain information for the network structure is observed. %while
%at the same time people's group activities may be indicative of the unseen connections.
%while again, more precise information for the network structure is manifestated in different ways. 
For example, we may know friendship links as appear in an online social network,
but we do not necessarily know the strength of those links. %, e.g., 
%some links may correspond to close friends and associates, 
%while others may correspond to remote acquaintances.
%In this example, observing how different groups of people interact and collaborate
%can be used to infer more detailed information about the existing type of links.
In such cases, 
where the network structure is not available, 
the fundamental question is to use manifestations of this hidden structure in order to reconstruct it.
\fi 

A different motivating scenario for our problem
is encountered when trying to characterize microbial communities, 
in computational biology.
Microbial species form symbiotic communities in different environments, 
such as different sites of the human body as well as the environment, 
such as the deep biosphere. 
Microbial communities are understood to be important players in their respective habitat, 
yet their structure and function is currently not well understood. 
Recent advances is DNA sequencing technology has now enabled 
a more detailed study of microbial communities. 
Analyzing the data can help us understand which species are working in symbiosis and which are 
in competition with each other.

Both of the previous scenarious
are examples in which the network structure is not available,
yet the fundamental question is to use manifestations of this hidden structure 
in order to reconstruct it.
We refer to this general class of data-mining problems as \emph{network-reconstruction} problems.


\iffalse
For example, a popular line of work 
focuses on the problem of inferring \emph{influence} in social networks~\cite{Anagnostopoulos:2008tj,Barbieri:2013bh,daneshmand14estimating,Du:2012ud,GomezRodriguez:2010ul,Gomez-Rodriguez12submodular,Goyal:2010uo,terzi09finding,Saito:2008,su2014structured}.
In this family of problems 
the input consists of actions performed by the network actors, 
e.g., the time of adoption of a product, 
and the goal is to estimate the social influence along each link of the network.
Another example is the case of 
\emph{link-prediction} problems~\cite{barbieri14who,gursun12who,hsieh12low,lichtenwalter10new,liben07link}. 
In this case, the input consists of a subset of network edges 
(partial or uncertain information about the network) 
and the goal is to identify missing edges or classify observed edges into different types. 

\begin{figure}
\centering
\includegraphics[width=0.95\columnwidth]{introfigure.pdf}	
\caption{\label{figure:intro}Reconstructing a network from a collection of sets.
In this case, in the reconstructed network, 
each of the input sets induces a subgraph of density at least~$2/3$.}
\vspace{3mm}
\end{figure}
\fi


\spara{Our problem:} The exact formulation of a network-re\-con\-struc\-tion problem depends on
the available information about the network and what we called manifestation of network structure.
In this paper, we consider a new class of network-reconstruction problems. 
The input consists of an underlying set of vertices $V$
and a collection $\sets = \{S_1,\ldots ,S_\ell\}$ of subsets of $V$.
The goal is to construct a \emph{sparse} graph $G$ in which the subgraphs
induced by the sets $S_i$ satisfy certain \emph{connectedness} properties.
We call this general problem the {\setnetworkprb} problem. 
An illustration of the problem we consider, in the form of input/output, 
is given in Figure~\ref{figure:intro}.

Our problem setting has many different applications. 
In social networks the input sets may correspond to groups of individuals who have collectively 
participated in various activities.
In collaboration networks, 
the input sets may correspond to teams of experts who
have successfully worked together on different projects. 
In these examples, the goal is to construct a parsimonious graph in which the individuals or 
experts who participate in the same groups are well connected.
As another application, in the design of computer networks, 
the input sets may correspond to sets of computer nodes for which we set certain connectedness requirements. 
Then, the goal is to construct the graph with the least number of links that satisfies those requirements.

The objective of minimizing the number of edges of the reconstructed network 
is a \emph{parsimony requirement}, 
and expresses the fact that real-world networks tend to be sparse.
It also implies that the problem we formulate can be seen as a
\emph{network-sparsification} operation. 
Namely, 
even if the network structure is known, 
we can still use our methods to identify a sparse subnetwork that satisfies certain connectedness requirements 
among specific subsets of vertices.
This gives us a concrete way to quantify the amount of \emph{redundancy} that exists in the network, 
with respect to those requirements.

% When the input sets correspond to teams of collaborators, then
% the question we ask is equivalent to finding the sparsest network 
% for which the observed collaborations are possible, 
% under a specific connectedness requirement.

Different connectedness properties lead to different instances of the {\setnetworkprb} problem.
We consider three properties (and combinations):
\emph{connectivity}, \emph{density}, and \emph{star containment}. 
While connectivity has been addressed by previous work~\cite{angluin13connectivity}, 
we are the first to introduce and study the other two properties, 
which define the {\densprb} and {\starprb} problems, respectively.

In the {\densprb} problem all input sets should induce dense subgraphs.  
% whose density is above a certain threshold.
This setting is motivated by regarding the input sets as {\em network communities}, 
which are typically assumed to be dense.
In the {\starprb} problem the requirement is that
for each input set should contain a star as a subgraph. 
The motivation for this requirement is that stars
have small diameter ($\Delta=2$), as well as
a central vertex that can assume a coordinating role.
Thus,
%  for certain applications, 
star-shaped graphs have low communication cost
and good coordination properties.

We view our work as a first step towards other 
network-reconstruction problems under different connectedness properties, 
such as, {\em small diameter}, 
{\em short paths}, 
{\em triangle density}~\cite{DBLP:conf/www/Tsourakakis15a},
{\em strong triadic closure}~\cite{DBLP:conf/kdd/SintosT14}, and more.
In this respect, our work opens exciting directions for future research
with respect to the study of those properties and the corresponding network-reconstruction problems.

In terms of technical results
we establish the computa\-tional complexity of both {\densprb} and {\starprb} problems,  
and we present approximation algorithms for solving them.
We validate our methods with experiments on real-world datasets, 
for which we compare the recon\-structed network with a ground-truth network.
% Our results show that the reconstructed networks have similar characteristics 
% with respect to the ground-truth networks, while using a smaller number of edges. 
Measuring precision and recall shows that
our algorithms recover a significant fraction of the ground-truth network. 
This is somewhat remarkable, 
as one would expect that the collection of input sets carries little information 
and under-specifies the problem of recovering all pairwise connections. 

The rest of the paper is organized as follows. 
We start by discussing the related work, in Section~\ref{section:related}, 
while in Section~\ref{sec:prel} we introduce our notation and formally define 
the general {\setnetworkprb} problem. 
In Sections~\ref{sec:density} and~\ref{sec:star} we study the problem for the two properties of interest,
density and star containment: 
in each case we establish the complexity of the problem and provide approximation algorithms. 
We experimentally validate our methods in Section~\ref{sec:exp}, 
while Section~\ref{sec:conclusions} is a short conclusion.

All the proofs are provided in the Appendix.

\section{Related work.}
\label{section:related}

To the best of our knowledge, we are the first ones to formally introduce and study the
the {\densprb} and {\starprb} problems.  
As a result, the problem definitions as well as the 
technical results and algorithms presented in this paper are novel.
However, our problems are clearly related to 
problems in \emph{network design} and \emph{hidden-network inference}.
%Below we summarize the existing work in these areas and we highlight 
%the key differences and connections between that work ours.

\spara{Network design problems:} 
At a high level, 
network-design problems consider a set of constraints 
%( e.g., reachability between certain pairs of vertices)
and ask to construct a minimum-cost network that satisfies those constraints~\cite{alon06general,angluin13connectivity,gupta12online,korach08complete,korach03clustering}. 
As in our case, cost is usually formulated in terms of the number of edges, 
or total edge weight.
Many different constraints have been considered in the literature: 
reachability between pairs of vertices, connectivity among subsets of vertices, cuts, flows, etc.
In some cases, as in this paper, offline problem versions are considered, 
where all the constraints are given in advance; 
in other cases, online versions are studied, where the constraints arrive in an online fashion.  
% In some cases the output network should be a subgraph of a given network, in other cases the output network can simply be a subgraph of the complete graph.

Among the existing work in network design, 
the most related to our paper is the work by Angluin {\etal}~\cite{angluin13connectivity}
and by Korach and Stern~\cite{korach03clustering,korach08complete}. 
Using the notation introduced in Section~\ref{sec:prel}, 
Angluin {\etal}\ essentially solve the {\setnetworkprb} problem 
with the $\indicator_{\connectivity}$ property. 
Our results on the {\densprb} problem and its variant on connected {\densprb}
(presented in Section~\ref{sec:density})
are largely inspired by the work of Angluin et al.
On the other hand, 
for the {\starprb} problem we need to introduce completely new techniques, 
as the submodularity property is not applicable in this case. 
Korach and Stern~\cite{korach03clustering,korach08complete} study the following problem: 
given a collection of sets, construct a minimum-weight {\em tree}
so that each given set defines a star in this tree.  
Clearly, this problem is related to the {\starprb} problem considered here, 
however, the tree requirement create a very significant differentiation: 
the problem studied by Korach and Stern is polynomially-time solvable, 
while {\starprb} is \NP-hard.
In terms of real-world applications, 
while tree structures are well motivated in certain cases (e.g., overlay networks), 
they are not natural in many other (e.g., social networks).

\spara{Inference of hidden networks:} 
The class of problems in this category
can be broadly defined as follows: 
given a set of observations originating from an underlying network 
infer the actual network structure.
The prototypical class of network-inference problems in machine learning
is the inference of Bayesian networks~\cite{hastie09elements}, 
where the goal is to learn conditional dependencies between latent variables. 
The problems studied in this paper 
consider a very different setting and are not directly related with this line of work.

Relevant, in terms of applications, 
is the recent work on inferring social influence~\cite{Anagnostopoulos:2008tj,Barbieri:2013bh,daneshmand14estimating,Du:2012ud,GomezRodriguez:2010ul,Gomez-Rodriguez12submodular,Goyal:2010uo,terzi09finding,Saito:2008}.
In the social-influence-inference problem, 
the observations stem from in\-di\-vid\-ual-level activities, e.g., 
adopting a product, performing an action, being infected by a virus, etc. 
The goal is to infer the most likely network that explains the observations.
The key difference between this line of work and ours is that our observations consist of sets of vertices, 
rather than activations of individual vertices. 
Additionally, in our setting there is no temporal information, 
which plays a critical role in the inference of influence networks.


Also related  
is the work of Liemhetcharat {\etal}~\cite{liemhetcharat11modeling,liemhetcharat12weighted}, 
which aims to infer team dynamics and interactions between robots. 
They consider teams as subsets of agents, as in our setting,
but they also consider performance scores for each given team. 
The goal is to infer the strength of the connections among the agents
as well as the ability level of each agent, 
so that the predicted structure is consistent with the observed team performance. 
The key differences with our work, is that we do not consider performance scores
and we do not assign  scores to vertices and our goal is network parsimony.
In addition, their problem formulation is probabilistic, while ours is combinatorial. 
To solve their problem, they follow an {\sc mcmc} approach, 
while we develop combinatorial algorithms with approximation guarantees.

\iffalse
\emph{Link prediction and characterization of edge types:} 
Problems that aim
to predict missing links~\cite{al2011survey,liben07link} 
% \cite{barbieri14who,gursun12who,hsieh12low,lichtenwalter10new,liben07link,wang2011human} 
or characterize the type of existing links~\cite{leskovec2010predicting, Sintos:2014jm,tang2012inferring}, can also
be viewed as network-reconstruction problems. 
However, these problems are very different than the ones we study in this paper, 
as they assume that a large part of the network is part of the input.
\fi


\iffalse
\para{Collaboration among professionals.}
An increasing number of clients are nowadays outsourcing their tasks to freelancers in virtual platforms, 
e.g., {\tt oDesk},\footnote{{\tt http://www.odesk.com}}
while amateurs and enthusiasts are delivering high-quality products developed 
by open-source initiatives.
In such fluid working environments it is crucial to be able to match the
right person with the right expertise to the right team.
Our network-inference framework contributes to this direction by
offering the capability to mine data from existing collaborations among professionals, 
and learn the structure of the underlying cooperation network---who can work efficiently with whom---which can be used to build skilled and effective teams.

\para{Cooperation among intelligent autonomous agents.}
Cooperation is encountered not only among humans, but also among
intelligent autonomous agents, such as robots or software components. 
With the upcoming {\em Internet of Things} revolution, an
very large number of devices and systems,  
covering a variety of protocols and domains, will be interconnected. 
Those autonomous agents will be expected to cooperate with each other.
Thus, it is crucial to be able to process the data produced by the
existing cooperations of groups of agents and draw conclusions
regarding their interaction dynamics, compatibility scores, and
synergy potential.
A first step to this direction was recently taken by 
Liemhetcharat et al.\ who addressed the problem of learning {\em synergy graphs} of
autonomous agents~\cite{Liemhetcharat:2014ju}.

\smallskip
As in the case of inferring social-influence networks, 
and as in the case of inferring missing edges and edge types, 
in order to be able to formulate a well-defined inference problem 
we need to make assumptions tying the observed collaborations with the underlying network structure.
For this purpose, we employ {\em connectivity} requirements.
Namely, we assume that observed collaborations correspond to tightly connected subgraphs in the network.
Furthermore, if performance scores are provided for the observed collaborations, 
we assume that these scores are translated to connectivity measures in the network.
We study three connectivity measures:
connectivity, density, and small diameter. 
The first measure has been addressed by previous work~\cite{angluin13connectivity}, 
while the latter two measures are considered for first time in this work.
For the diameter measure we focus in the case that the diameter is equal to two, 
implying that each observed collaboration should be covered by a ``star'' graph, 
namely for each observed collaboration there should be a central leader.

Our network-inference problem is then formulated as follows:
{\em 
Given a set of observed collaborations, 
and a connectivity measure that models who collaborations are formed, 
find the network with minimum number of edges 
so that the connectivity requirement is satisfied for all observed collaborations.
}


\todo{\bf outline of our theoretical and experimental results and contributions}
\fi	


==> s2n-prel.tex <==
\section{General problem definition}
\label{sec:prel}

% In this section, we introduce our notation, and formally define the problem we address, {\setnetworkprb}.

In this section we give a high-level description of our problem.
Since our goal is to form a network from a collection of sets, 
we call our general problem {\setnetworkprb}. 
Before introducing the problem we describe our setting,  
and the notation we will use throughout the paper.

We consider a set $V$ of $n$ vertices.
Our input consists of a collection of $\ell$ sets $\sets = \{S_1,\ldots ,S_\ell\}$ over $V$, 
i.e., $S_i\subseteq V$. 
% The sets in $\sets$ represent the observed collaborations 
% from which we want to infer the underlying network structure.   
We assume that every vertex in $V$ appears in at least one set in $\sets$, 
that is, $\cup_{i=1}^\ell S_i=V$.
Without loss of generality, we also consider as part of the input, 
a \emph{feasibility network} $G_0=(V,E_0)$. 
The set $E_0$ represents candidate edges that can be included 
in the reconstructed network. 
In other words, if $G=(V,E)$ is the {\em output network}, 
we require $E\subseteq E_0$. 
If there is no information regarding the feasibility network $G_0$
we just assume that it is the \emph{complete graph}.
% For simplicity of presentation we are assuming that $G_0$ is the complete graph, 
% however, our results are applicable for any given network $G_0$.

\spara{Graph properties:}
Given a graph $G=(V,E)$ and a set of vertices $S\subseteq V$, 
we use $E(S)$ to denote the edges of $E$ that have both endpoints in $S$. 
Accordingly, $G(S)=(V,E(S))$ is the subgraph of $G$ \emph{induced} by~$S$.
For a given graph $G$ and a collection of subsets of vertices $\sets = \{S_1,\ldots ,S_\ell\}$, 
we are interested whether the graph $G$ satisfies a certain property $\Property$
for each set $S_i\in \sets$. 
% We consider graph properties such as connectivity or density.
We say that $G$ \emph{satisfies property $\Property$ with respect to} $S_i$ 
if the induced subgraph $G(S_i)$ satisfies property $\Property$. 
We write $\indicator_\Property(G,S_i)=1$ 
to denote the fact that $G(S_i)$ satisfies property $\Property$, 
while $\indicator_\Property(G,S_i)=0$, otherwise.
In this paper, we consider three graph properties: 
($i$) \emph{connectivity}, denoted by $\connectivity$; 
($ii$) \emph{density}, denoted by $\density$; and 
($iii$) \emph{star containment}, denoted by $\stars$.
The corresponding indicator functions are denoted by 
$\indicator_\connectivity$, 
$\indicator_{\density\ge\alpha_i}$, 
and 
$\indicator_{\stars}$.

\note[Aris]{The above paragraph is very terse. Motivation for the three properties should come in the intro.}

\iffalse
The connectivity property requires that each set $S_i$
induces a connected subgraph.
The density property requires that each set $S_i$ 
induces a subgraph of density at least $\alpha_i$.
The star property requires that each set $S_i$ induces a graph that contains a star. 
This property is motivated by the more general case of having subgraphs with small diameter. 
We focus on the star property as it is interesting in its own right and yet algorithmically challenging.
\fi 

\spara{Problem definition:}
We are now ready to define the general problem that we study in this paper.

\begin{problem}[{\setnetworkprb}]
\label{problem:general}
Consider a set of vertices $V$, 
a feasi\-bi\-lity network $G_0=(V, E_0)$ over $V$, 
and a graph property $\Property$.
Given a collection of $\ell$ subsets of vertices
$\sets = \{S_1,\ldots, S_\ell\}$, 
we want to construct a network $G = (V, E)$, such that, 
($i$) $E \subseteq E_0$; 
($ii$) $\indicator_\Property(G,S_i) = 1$, for all $S_i\in\sets$;  
and 
($iii$) the number of edges $|E|$ is minimized. 
\end{problem}
% In other words, {\setnetworkprb} asks to construct a network $G$, 
% which has subgraphs satisfying certain properties,
% and it has the minimum possible number of edges.  

 
Clearly, the complexity and the solutions for Problem~{\ref{problem:general}} depend on the exact property $\Property$ 
used in the problem definition.
Angluin {\etal}~\cite{angluin13connectivity} study the problem for the connectivity property.
i.e., they want to find a graph $G$ so that the subgraph induced by every set $S_i\in\sets$ is connected. 
% In their paper, 
They show that it is \NP-hard and provide a greedy algorithm with logarithmic approximation guarantee.
Here we study the {\setnetworkprb} problem for the density and star properties.
We discuss the two problems in detail in the next sections. 
We show that both problems are \NP-hard 
and we provide approximation algorithms for solving them.



==> tables1.tex <==

\begin{table*}[ht!]
	\caption{Number of edges in the inferred network, obtained by different approaches. Column $E_0$ contains number of edges in the initial network, other columns contain number of edges in the inferred network by corresponding algorithm. \densprb~ problem was solved using different values of parameter $\epsilon$.}
	\centering
	\begin{tabular}{l rrrrrrrrrrrr}
	\toprule
	Name && $E$ &\matching & $\starrandom$ &&
	\multicolumn{3}{c}{$\densitygreedy$} &&
	\multicolumn{3}{c}{$\densityrandom$}\\
	\cmidrule{7-9}
	\cmidrule{11-13}
	%\toprule
	&&&&&&$\epsilon=0.5$&$\epsilon=0.7$&$\epsilon=1.0$&&$\epsilon=0.5$&$\epsilon=0.7$&$\epsilon=1.0$\\
	\midrule  
	Amazon1  && 11606 & 7010 & 8657 && 3801 & 4819 & 7597 && 5502 & 6801 & 9746\\
	Amazon2 && 25129 & 16781 & 21738 && 8587 & 10630 & 16604 && 13803 & 16704& 23642\\
	DBLP1 && 12801 & 5167 & 5591 && 4894 & 6983 & 10880 && 5484 & 7552 & 11355\\
	DBLP2 && 27687 & 10333 & 11272 && 9892 & 14157 & 22123 && 11110 & 15401 & 23097\\
	Youtube1 && 38294 & 6295 & 7177 &&  3378 & 4580 & 7529 && 4485 & 5833 & 8750\\
	Youtube2 && 72215 & 12875 & 14673 && 6836 & 9055 & 14837 && 9191 & 11628 & 17456\\
	
	\bottomrule
	\end{tabular}
	\label{tab:edges}
	
\end{table*}

\begin{table*}[ht!]
	\caption{Characteristics of the inferred network. Column $d_{avg}$ contains average degree; $D_{90\%}$ contains effective diameter, found as $0.9\%$-quantile of finite shortest paths lengths; $p$~-- is a median of the finite shortest paths lengths. \densprb~ problem was solved using different values of parameter $\epsilon$.}
	\centering
	\begin{tabular}{l rrrrrrrrrrrrrrrr}
		\toprule
		Name &&
		\multicolumn{3}{c}{$\matching$}&&
		\multicolumn{3}{c}{$\densitygreedy$, $\epsilon=0.5$} &&
		\multicolumn{3}{c}{$\densitygreedy$, $\epsilon=0.7$} &&
		\multicolumn{3}{c}{$\densitygreedy$, $\epsilon=1.0$}\\
		\cmidrule{3-5}
		\cmidrule{7-9}
		\cmidrule{11-13}
		\cmidrule{15-17}
		%\toprule
		&& $d_{avg}$&$D_{90\%}$&$p$&& $d_{avg}$&$D_{90\%}$&$p$&& $d_{avg}$&$D_{90\%}$&$p$&& $d_{avg}$&$D_{90\%}$&$p$\\
		\midrule  
		Amazon1  && 2.805 & 13 & 9 && 1.521 & 32 & 21  && 1.930 & 24 & 17  && 3.039 & 16 & 11 \\
		Amazon2 && 3.356 & 18 & 10 && 1.717 & 36 & 24  && 2.126 & 25 & 17 && 3.321 & 17 & 12 \\
		DBLP1 && 2.065 & 19 & 14 && 1.956 & 31 & 16 && 2.791 & 24 & 15 && 4.349 & 18 & 13 \\
		DBLP2 && 2.066 & 19 & 14 && 1.978 & 31 & 19 && 2.831 & 22 & 15 && 4.424 & 17 & 13 \\
		Youtube1 && 2.518 & 9 & 6 && 1.351 & 13 & 7&& 1.832 & 11 & 7  & & 3.012 & 9 & 6\\
		Youtube2 && 2.575 & 9 & 6 && 1.367 & 11& 8 && 1.811 & 10& 7 && 2.967 & 9& 7\\
		
		\bottomrule
	\label{tab:result-characteristics}
	\end{tabular}	
\end{table*}

\begin{table*}[ht!]
	\caption{Accuracy of the inferred network measured against the ground-truth network. Columns $P$, $R$, $F_1$ contain values of precision, recall and $F_1$-measure correspondingly. \densprb~ problem was solved using different values of parameter $\epsilon$.}
	\centering
	\begin{tabular}{l rrrrrrrrrrrrrrrr}
		\toprule
		Name &&
		\multicolumn{3}{c}{$\matching$}&&
		\multicolumn{3}{c}{$\densitygreedy$, $\epsilon=0.5$} &&
		\multicolumn{3}{c}{$\densitygreedy$, $\epsilon=0.7$} &&
		\multicolumn{3}{c}{$\densitygreedy$, $\epsilon=1.0$}\\
		\cmidrule{3-5}
		\cmidrule{7-9}
		\cmidrule{11-13}
		\cmidrule{15-17}
		%\toprule
		&& $P$&$R$&$F_1$&&$P$&$R$&$F_1$&&$P$&$R$&$F_1$&&$P$&$R$&$F_1$\\
		\midrule  
		Amazon1  && 0.590 & 0.357 & 0.445 && 0.763 & 0.250 & 0.376 && 0.718 & 0.298 & 0.421 && 0.649 & 0.425 & 0.513 \\
		Amazon2 && 0.606 & 0.405 & 0.485 && 0.836 & 0.285 & 0.426 && 0.790 & 0.334 & 0.469 && 0.700 & 0.462 & 0.557 \\
		DBLP1 && 0.603 & 0.243 & 0.347 && 0.716 & 0.273 & 0.396 && 0.697 & 0.380& 0.492 && 0.660 & 0.561 & 0.606 \\
		DBLP2 && 0.612 & 0.228 & 0.333 && 0.730 & 0.261 & 0.384 && 0.707 & 0.361 & 0.478 && 0.672 & 0.537 & 0.597 \\
		Youtube1 && 0.506 & 0.083 & 0.143 && 0.683 & 0.060 & 0.110 && 0.625 & 0.074 & 0.133 & & 0.564 & 0.110 & 0.185 \\
		Youtube2 && 0.554 & 0.099 & 0.168 && 0.745 & 0.070 & 0.128 && 0.685 & 0.086 & 0.152 && 0.604 & 0.124 & 0.206\\
		
		\bottomrule
	\end{tabular}
	\label{tab:precision-recall}	
\end{table*}

\begin{table*}[ht!]
	\caption{Running time of the algorithms. Time is given in seconds. Algorithms \matching~and \stargreedy, as well as \densitygreedy~and \densitysort, share the same preprocessing stages, its running time is given correspondingly in columns $TP_{star}$ and $TP_{dense}$. Columns \matching, \stargreedy, \densitygreedy~and \densitysort~contain running time of the algorithms without preprocessing phase.}
	\centering
	\setlength{\tabcolsep}{0pt}
	\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l rrrrrrrrrrrrr}
		\toprule
		Name && $TP_{star}$ &
		\matching & \stargreedy &&
		$TP_{dense}$ &
		\multicolumn{3}{c}{\densitygreedy} &&
		\multicolumn{3}{c}{\densitysort}\\
		\cmidrule{8-10}
		\cmidrule{12-14}
		%\toprule
		&&&&&&&$\epsilon=0.5$&$\epsilon=0.7$&$\epsilon=1.0$&&$\epsilon=0.5$&$\epsilon=0.7$&$\epsilon=1.0$\\
		\midrule  
		Amazon1  && 0.013 & 0.313 & 0.167 &&15.30& 0.202 & 0.226 & 0.217 && 0.062 & 0.071 & 0.085\\
		Amazon2 && 0.027 & 0.978 & 0.662 &&224.51& 0.700 & 0.988 & 0.622 && 0.163 & 0.312&  0.209\\
		DBLP1 && 0.004 & 0.071 & 0.034 &&11.07& 0.167 & 0.194 & 0.207 && 0.047 & 0.061 & 0.077\\
		DBLP2 && 0.009 & 0.172 & 0.089 &&102.09& 0.420 & 0.443 & 0.480 && 0.102 & 0.130 & 0.149\\
		Youtube1 && 0.007 & 0.082 & 0.039 &&16.45&  0.354 & 0.227 & 0.236 && 0.069 & 0.056 & 0.069\\
		Youtube2 && 0.012 & 0.267 & 0.132 &&99.57& 0.369 & 0.380 & 0.301 && 0.157 & 0.172 & 0.160\\
		
		\bottomrule
	\end{tabular*}
	\label{tab:time}
\end{table*}



==> tmp-algos.tex <==
In this paragraph, we discuss two algorithms for the {\starprb}.  The common characteristic of both the algorithms is that they translate the diameter requirement into a ``star" requirement
where in the output graph $G=(V,E)$ all the subgraphs defined by the edges
in $E(S_i)$ are stars with one node being the central nodes of the star
and the rest being connected to this central node.


\subsubsection{The {\matching} algorithm}
In order to introduce the {\matching} algorithm, we first introduce the 
\emph{directed} variant of the {\starprb} as follows:
\begin{problem}[\distarprb]
Given a graph $G_0 = (V, E_0)$, $\ell$ and $\ell$
subsets $\sets = \{S_1,\ldots, S_\ell\}$, find a \emph{directed} graph 
$G_d = (V, D)$
such that  $\abs{D}$ is minimized and for $(x\rightarrow y)
\in E_d$ either $(x, y) \in E_0$ or $(y, x) \in E_0$ such that for each $S_i$ there
is a node $c_i \in S_i$ having edge $(c_i \rightarrow x)$ for the remaining nodes $x \in S_i$.
\end{problem}

The main difference between the {\distarprb} and the {\starprb} problems is that the former
outputs a \emph{directed} graph $G_d$. 
This graph has the following property with respect to the
sets $\sets$; each set $S_i$ induces a directed star in $G_d$, where one of the nodes  
$c_i\in S_i$ is the ``center" of this star and there are \emph{directed} edges $(c_i\rightarrow x)\in D$ for every $x\in S_i$.

The relationship between the {\starprb} and the {\distarprb} problems is best summarized in 
the following lemma.

\begin{proposition}\label{prop:relationship}
If $G^\ast = (V,E^\ast)$ is the optimal solution to the {\starprb} and 
$G^\ast_d=(V,D^\ast)$ is the optimal solution to the {\distarprb} problems for the same
input, then $\abs{D^\ast}\leq 2\times \abs{E^{\ast}}$.
\end{proposition}
Intuitively, this is true because in $|E^\ast|$ we count undirected edges, which 
are counted potentially twice in both directions in $|D^\ast|$.
This essentially means, that if we had an algorithm that solved optimally {\distarprb},
then we could simply translate all directed edges in $G^\ast_d=(V,D^\ast)$ into undirected,
omit the duplicates and obtain a solution to  {\starprb} which is within a factor
$2$ of the optimal solution.

However, the problem is that the {\distarprb} problem is NP-Complete~\footnote{The proof of Proposition~\ref{prop:starhardness} can be modified slightly to show that}. Therefore, 
first we need to design an approximation algorithm for {\distarprb} and then translate 
the solution of this algorithm into a solution of {\starprb} as we described above.
We do that in the next paragraph.


\spara{An algorithm for the {\distarprb} problem:}
First, we observe that {\distarprb} can be viewed as a {\hyperprb} problem, 
where given a
a universe $X$, a collection of hyperedges $\mathcal{H} = \{H_1,\dots H_t\}$,
$H_i \subseteq X$, and score function $\funcdef{c}{H}{\Reals}$, 
we seek to find a set of disjoint hyperedges $\mathcal{O}$
maximizing the total score $\sum_{H_i\in \mathcal{O}} c(H_i)$.\footnote{Ties are resolved by taking the largest set.}

The mapping from the {\distarprb} to the {\hyperprb} problem is done as follows:
We set universe to be $\sets$.  Given a subset $\mathcal{C} \subseteq \sets$, let us
define $\intersection(\mathcal{C})$ and $\union(\mathcal{C})$ 
to be the intersection and union of members in $\mathcal{C}$,
respectively. Let us construct a set of hyperedges as
\[
	\mathcal{H} = \left\{H \mid H \subseteq \sets \text{ and } \intersection(H) \ne \emptyset\right\}.
\]
and the scores
\[
	c(H) = 1 - \abs{H} + \sum_{v \in \union(H)} \abs{\set{i \mid v \in S_i \in H}} - 1.
\]
This is the instance of the {\hyperprb} problem we will be focusing on and this is the instance
we will be considering for the rest of the paragraph.
We should point out that $\mathcal{H}$ can be of exponential size. However, we will avoid
any problems as we will never construct this set explicitly. %, see Section~\ref{sec:staralg}.

Now we can show that the optimal solution $\mathcal{O}$ to the instance of 
 {\hyperprb} we created above can be used to construct the optimal solution to the 
 {\distarprb} problem.  This is described in the following proposition:

\begin{proposition}\label{prop:optimal}
Let $\mathcal{O}$ be the optimal solution
for {\hyperprb} and $D_\mathcal{O}$
be union of directed stars, each star having a center in $\intersection(H)$
and directed edges towards nodes in $\union(H)$ for every $H \in \mathcal{O}$. 
If 
$D^\ast$ is the optimal solution to the 
{\distarprb} problem, then $D^\ast=D_\mathcal{O}$ 
and 
\[
	 \abs{D^\ast} = \abs{D_\mathcal{O}}=\sum_{S_i\in\sets}(|S_i| - 1)  - \sum_{H \in \mathcal{O}} c(H).
\]
\end{proposition}

To prove the proposition we will use the following lemma which we will state without
the proof.


\begin{lemma}
\label{lem:star}
Let $D_\mathcal{T}$ 
be a union of directed edges defined by a set of stars $\mathcal{T} = \set{T_i}$, each $T_i$
spanning an $S_i\in\sets$. Define $d(e) = \abs{\set{i \mid e \in T_i}} - 1$.
Then
\[
	\abs{D_\mathcal{T}} = \sum_{S_i\in \sets}(|S_i| - 1) - \sum_{e \in D_\mathcal{T}} d(e).
\]
\end{lemma}

The first term sums over all sets and is a trivial upper bound
solution, where each star covers exactly one set. This term is constant, denote
is as $C$. The second term corrects the first by taking into account edges
that have been counted multiple times.

Now we are ready to prove Proposition~\ref{prop:optimal}.
\begin{proof}
Let $D^\ast$ be optimal solution to {\distarprb}.
Since $\mathcal{H}$ contains all $S_i$'s as single groups, every set $S_i$ in included in
some $H \in \mathcal{O}$. Hence, $D_\mathcal{O}$  
is a feasible solution for {\distarprb} and $\abs{D^\ast} \leq \abs{D_\mathcal{O}}$.

Due to its optimality, $D^\ast$ is a union of stars $\set{T_i}$, each $T_i$ spanning
$S_i$.  Define a partition $\mathcal{P}$ of $\mathcal{S}$ by grouping each
$S_i$ sharing the same star center. This is a feasible solution to {\hyperprb}.
Moreover, $c(H) = \sum_{(x\rightarrow y) \in D^\ast} d(e)$, where $x$ is the center of a star
spanning the sets in $H \in \mathcal{P}$. Since similar result holds for $\mathcal{O}$,
Lemma~\ref{lem:star} and the optimality of $\mathcal{O}$ imply
\[
	\abs{D^\ast} = C - \sum_{H \in \mathcal{P}} c(H) \geq C - \sum_{H \in \mathcal{O}} c(H) = \abs{D_\mathcal{O}},
\]
which completes the proof.
\end{proof}

Consider a greedy algorithm,  which constructs a solution 
to the {\hyperprb} problem as follows: it adds the hyperedges to $\mathcal{U}$
one by one to maximize the total score $\sum_{H_i\in \mathcal{U}} c(H_i)$ on each step
while keeping $\mathcal{U}$ disjoint. The algorithm terminates, when no more hyperedges
can be added. We call this greedy algorithm the {\hypergreedy} algorithm.

\note{This should be known result, I am not sure which citation to use}
\note[ET]{Add citation}

\begin{proposition}\label{prop:kapprox}
Let $\mathcal{U}$ be the resulting set given by
the {\hypergreedy} algorithm, and let $\mathcal{O}$ be the optimal solution for {\hyperprb}.
Then,
\[
	\sum_{H \in \mathcal{O}} c(H) \leq k \sum_{H \in \mathcal{U}} c(H),
\]
where $k = \max_{H \in \mathcal{H}} \abs{H}$.
\end{proposition}

This means that the {\hypergreedy} algorithm is a $k$-approximation algorithm for 
the {\hyperprb} problem.  Propositions~\ref{prop:optimal} 
and~\ref{prop:kapprox} imply the following:

\begin{corollary}
\label{cor:dirbound}
Let $D^\ast$ be the optimal solution of {\distarprb}.
Let $\mathcal{U}$ be the greedy solution to the corresponding {\hyperprb} problem,
and let $D_\mathcal{U}$ be the corresponding edges (obtained as described in 
Proposition~\ref{prop:optimal}). Then,
\[
	\abs{D_\mathcal{U}} \leq \frac{k - 1}{k} C + \frac{1}{k}\abs{D^\ast},
\]
where $C = \sum_{S_i\in\sets} \left(\abs{S_i} - 1\right)$ 
and $k$ is the maximum number of sets in
$\sets$ that have a non-empty intersection.
\end{corollary}


\spara{Putting everything together:}
Now we are ready to put everything together into designing the {\matching} algorithm for 
the {\starprb} problem.  The pseudocode of {\matching} is shown in Algorithm~\ref{algo:matching}.  In the first step, the algorithm invokes {\hypergreedy}
and obtains and solution to the {\hyperprb}, as we described above.
This solution, is then translated into a solution to the {\distarprb} problem
using the transformation procedure explained in the body of Proposition~\ref{prop:optimal}.
Finally, the solution to {\distarprb} is translated into a solution to the {\starprb}
by transforming each directed edge in $D_\mathcal{U}$ into an undirected edge and removing
duplicates.

\begin{algorithm}
	\caption{The {\matching} algorithm for {\starprb}.}
	\label{algo:matching}
	%\begin{algorithmic}
		\KwData{$G_0=(V,E_0)$ and $\sets = \{S_1,\ldots , S_\ell\}$}
		\KwResult {Graph $G=(V,E)$ such that $E(S_i)$ defines a subgraph of diameter $2$ for all $i\in 1,\ldots ,\ell$.} 
	
		{{\bf Step 1: }$\mathcal{U}=$ {\hypergreedy}$(\sets)$}\;
		{{\bf Step 2: }$D_\mathcal{U} = \texttt{H2D}(\mathcal{U})$}\;
		{{\bf Step 3: }$E = \texttt{D2E}(D_\mathcal{U})$}\;
		%\tcc{update search space of $\mathcal{H}$ to keep $\mathcal{U}$ disjoint}
		\Return $G=(V,E)$\;
	%\end{algorithmic}
\end{algorithm}

We have the following result with respect to the performance of
{\matching}.
\begin{proposition}
\label{prop:undirbound}
Let $E^\ast$ be the optimal solution of {\starprb}.
Let $\mathcal{U}$ be the greedy solution to the corresponding {\hyperprb} problem,
and let $E$ be the output of the {\matching} algorithm. Then,
\[
	\abs{E} \leq \frac{k - 1}{k} C + \frac{2}{k}\abs{E^\ast},
\]
where $C = \sum_{S_i\in\sets} (\abs{S_i} - 1)$ and $k$ is the maximum number of sets in
$\sets$ that have a non-empty intersection.
\end{proposition}

\begin{proof}
Let $D^\ast$ be the directed version of $E^\ast$, where each edge is oriented from a
star center, possibly doubling edges whenever needed. Each undirected edge
may spawn at most 2 directed edges, consequently, $\abs{E\ast} \leq \abs{D^\ast}$.
Since, $D^\ast$ is a feasible solution for {\distarprb}, Corollary~\ref{cor:dirbound}
proves the statement.
\end{proof}


\iffalse
\note[ET]{Can we add here a statement potentially connecting $\set{E}$ and $\set{E'}$ without
having the text in between so that it become clearer to the readers why we introduce this problem?}

For the rest of the discussion we will describe an algorithm for solving the {\distarprb}
problem and then show that this is a good algorithm for the {\starprb} as well.

\note[ET]{Citation to hyperedge matching problem?}

For this we first observe that {\distarprb} can be viewed as a {\hyperprb} problem, 
where given a
a universe $X$, a collection of hyperedges $\mathcal{H} = \{H_1,\dots H_t\}$,
$H_i \subseteq X$, and score function $\funcdef{c}{H}{\Reals}$, 
we seek to find a set of disjoint hyperedges $\mathcal{O}$
maximizing the total score $\sum_{H_i\in \mathcal{O}} c(H_i)$.\footnote{Ties are resolved by taking the largest set.}

The mapping from the {\distarprb} to the {\hyperprb} problem is done as follows:
We set universe to be $\sets$.  Given a subset $\mathcal{C} \subseteq \sets$, let us
define $\intersection(\mathcal{C})$ and $\union(\mathcal{C})$ 
to be the intersection and union of members in $\mathcal{C}$,
respectively. Let us construct a set of hyperedges as
\[
	\mathcal{H} = \left\{H \mid H \subseteq \sets \text{ and } \intersection(H) \ne \emptyset\right\}.
\]
and the scores
\[
	c(H) = 1 - \abs{H} + \sum_{v \in \union(H)} \abs{\set{i \mid v \in S_i \in H}} - 1.
\]
We should point out that $\mathcal{H}$ can be of exponential size. However, we will avoid
any problems as we will not construct this set explicitly, see Section~\ref{sec:staralg}.

Now we can show that the optimal solution $\mathcal{O}$ to the instance of 
 {\hyperprb} we created above can be used to construct the optimal solution to the 
 {\distarprb} problem.  This is described in the following proposition:

\begin{proposition}\label{prop:optimal}
Let $\mathcal{O}$ be the optimal solution
for {\hyperprb}. Define $E^\ast$ to be union of stars, each star having a center in $\intersection(H)$
and spanning $\union(H)$ for every $H \in \mathcal{O}$. Then $E^\ast$ is 
the optimal solution
for {\distarprb} with cardinality 
\[
	 \abs{E^*} = \sum_{S_i}(|S_i| - 1)  - \sum_{H \in \mathcal{O}} c(H).
\]
\end{proposition}

To prove the proposition we will use the following lemma which we will state without
the proof.

\note[ET]{I am a little bit confused about the lemma. How do you obtain the $T_i$'s? Are they 
directed or undirected?. }

\begin{lemma}
\label{lem:star}
Let $E'$ be a union of stars $\set{T_i}$, each $T_i$
spanning $S_i$. Define $d(e) = \abs{\set{i \mid e \in T_i}} - 1$.
Then
\[
	\abs{E'} = \sum_{S_i}(|S_i| - 1) - \sum_{e \in E'} d(e).
\]
\end{lemma}

The first term sums over all sets and is a trivial upper bound
solution, where each star covers exactly one set. This term is constant, denote
is as $C$. The second term corrects the first by taking into account edges
that have been counted multiple times.

Now we are ready to prove Proposition~\ref{prop:optimal}.
\begin{proof}
Let $E'$ be the solution to \distarprb.
Since $\mathcal{H}$ contains all $S_i$ as single groups, every set $S_i$ in included in
some $H \in \mathcal{O}$. Hence, $E^*$ is a feasible solution and $\abs{E'} \leq \abs{E^*}$.

Due to the optimality $E'$ is a union of stars $\set{T_i}$, each $T_i$ spanning
$S_i$.  Define a partition $\mathcal{P}$ of $\mathcal{S}$ by grouping each
$S_i$ sharing the same star center. This is a feasible solution to \hyperprb.
Moreover, $c(H) = \sum_{(x, y) \in E'} d(e)$, where $x$ is the center of a star
spanning the sets in $H \in \mathcal{P}$. Since similar result holds for $\mathcal{O}$,
Lemma~\ref{lem:star} and the optimality of $\mathcal{O}$ imply
\[
	\abs{E'} = C - \sum_{H \in \mathcal{P}} c(H) \geq C - \sum_{H \in \mathcal{O}} c(H) = \abs{E^*},
\]
which completes the proof.
\end{proof}


\subsubsection{Greedy algorithm}\label{sec:staralg}
Consider a greedy algorithm, given in Algorithm~\ref{alg:greedy}, which adds the hyperedges to $U$
one by one to maximize the total score $\sum_{H_i\in U} c(H_i)$ on each step
while keeping $U$ disjoint. The algorithm terminates, when no more hyperedges
can be added. 

\begin{algorithm}
	\caption{Greedy algorithm for \hyperprb problem}
	\label{alg:greedy}
	%\begin{algorithmic}
		\KwData{Set of hyperedges $\mathcal{H}$}
		\KwResult {Hyperedge matching $\mathcal{U}$} 
		%\Require Set of hyperedges $H$
		{ $\mathcal{U} \define \emptyset$}\;
		\While{$\mathcal{H} \ne \emptyset$}{		
		{$H^*  \define  \arg\max_{H \in \mathcal{H}} {c(H)}$}\;
		$\mathcal{U} \define \mathcal{U}\cup H^*$\;		
		$\mathcal{H}  \define  \{H \in \mathcal{H} \mid H \cap H^* =\emptyset\}$\;
		%\tcc{update search space of $\mathcal{H}$ to keep $\mathcal{U}$ disjoint}
		}
		\Return $\mathcal{U}$\;
	%\end{algorithmic}
\end{algorithm}

\note{This should be known result, I am not sure which citation to use}
\begin{proposition}
Let $\mathcal{U}$ be the resulting set given by
the greedy algorithm, and let $\mathcal{O}$ be the optimal solution for \hyperprb.
Then
\[
	\sum_{H \in \mathcal{O}} c(H) \leq k \sum_{H \in \mathcal{U}} c(H),
\]
where $k = \max_{H \in \mathcal{H}} \abs{H}$.
\end{proposition}

\note{How to obtain edges from matching}


\begin{corollary}
\label{cor:dirbound}
Let $E'$ be the optimal solution of \distarprb.
Let $\mathcal{U}$ be the greedy solution to the corresponding \hyperprb problem,
and let $E^*$ be the corresponding edges. Then
\[
	\abs{E^*} \leq \frac{k - 1}{k} C + \frac{1}{k}\abs{E'},
\]
where $C = \sum \abs{S_i} - 1$ and $k$ is the maximum number of sets in
$\mathcal{S}$ that have a non-empty intersection.
\end{corollary}

\note{How to obtain undirected edges from matching}

\begin{corollary}
\label{cor:undirbound}
Let $E'$ be the optimal solution of \starprb.
Let $\mathcal{U}$ be the greedy solution to the corresponding \hyperprb problem,
and let $E^*$ be the corresponding edges. Then
\[
	\abs{E^*} \leq \frac{k - 1}{k} C + \frac{2}{k}\abs{E'},
\]
where $C = \sum \abs{S_i} - 1$ and $k$ is the maximum number of sets in
$\mathcal{S}$ that have a non-empty intersection.
\end{corollary}

\begin{proof}
Let $D'$ be the directed version of $E'$, where each edge is oriented from a
star center, possibly doubling edges whenever needed. Each undirected edges
may spawn at most 2 directed edges, consequently, $\abs{D'} \leq \abs{E'}$.
Since, $D'$ is a feasible solution for \distarprb, Corollary~\ref{cor:dirbound}
proves the statement.
\end{proof}
\fi

\spara{Running time:}
The cost function $c(\cdot)$ is monotone with $c(H)\geq c(H')$ for $H' \subseteq H$, as the more sets are covered by the same star, the more
edges are reused. Thus, during each step the greedy algorithm considers only
hyperedges, which are not a proper subset of any hyperedge in $H$. 
\note{more discussion here, number of maximal sets is bounded by $\abs{V}$}



\subsubsection{The {\stargreedy} algorithm}
The {\stargreedy} algorithm again adopts the view of the output graph $G=(V,E)$
as a collection of stars, where each star corresponds to a set $S_i$ and 
for each set $S_i$ there is a node $c_i\in S_i$ that is the central node of the corresponding
star. With this view in mind, {\stargreedy} greedily tries to minimize the total number of 
distinct central nodes, with the hope that having stars with a lot of common
central nodes will result in fewer edges in the output graph.

Therefore, the {\stargreedy} algorithm starts
with $E=\emptyset$ and all sets $\sets = \{S_1,\ldots ,S_\ell\}$
being uncovered. At every iterate, 
the algorithm picks  node $c$ such that $c$
participates in the largest number of uncovered sets. 
Once $c$ is picked, then all edges $\{e(c,x)\mid c\in S_i\text{ and } x\in S_i \text{ and } S_i \text{ is uncovered}\} $ are added to $E$ and all sets $S_i$ that have the property that
$E(S_i)$ has diameter $2$ are marked as covered.  The algorithm terminates when 
there are no more uncovered sets.



\note[ET]{Running time}



==> triad.tex <==
\iffalse % not used in the paper
\section{Triadic closure}

Assume that edges are typed, strong (\strong) and weak (\weak).
We observe the network structure (edges) but we do not know the edge
types.
We are also given teams $T_1,\ldots, T_k\subseteq V$.

We want to infer the edge types, and we consider the following
principles.
\begin{enumerate}
\item
A triple with two strong edges and a non-edge violates the 
{\em strong triadic closure}  property (STC).
We want to minimize the number of STC violations.
\item
The given teams should be \strong-connected, 
meaning that each pair of vertices in a team should be connected via a
path of edges of type \strong.
\end{enumerate}

We can now formulate the edge inference problem by taking into account
the above properties. 

\begin{problem}
\label{problem:stc}
We are given a graph $G=(V,E)$ 
and a set of teams 
$T_1,\ldots, T_k\subseteq V$.
The objective is to infer the type of edges of $E$ as \strong\ or \weak, 
so that all given teams are \strong-connected and the number
of STC violations is minimized.
\end{problem}

The problem is interesting even when there is only one group, which is
equal to the whole set of vertices. 
In this case, we want to find a set of edges to label as strong so
that the whole graph is strongly connected, and the number of STC
violations is minimized.

\begin{observation}
Consider an \strong-connected graph $G$ that solves
Problem~\ref{problem:stc}. 
Then $G$ is a tree.
\end{observation}

\begin{proof}
Changing an edge type from \strong\ to \weak\ does not introduce
additional STC violations.
\end{proof}

\begin{proposition}
Problem~\ref{problem:stc} is \NP-hard. 
\end{proposition}

We will encode edge labelings by specifying the set of edges $X$ that are
labeled \strong, and assume that the rest of the edges $E\setminus X$
are labeled \weak.

Consider an edge labeling with \strong-edges $X$.
Define $\violations(X)$ to be the number of STC violations given by
the set of \strong-edges $X$.

\begin{proposition}
The function $\violations(X)$
 is {\em supermodular} with respect to
the set of \strong-edges $X$.
\end{proposition}

\begin{proof}
For an \strong-edge set $X$, and a node $u$ define 
$N_{X}(u) = \{ v \mid (u,v)\in X\}$
(the \strong-neighbors of $u$)
and 
$\overline{N}(u) = \{ v \mid (u,v)\not\in E\}$
(the non-neighbors or $u$).

For an \strong-edge set $X$ and an edge $e=(u,v)$
the number of additional STC violations introduced by labeling edge
$e$ as \strong\ is given by 
\[ 
\violations(X\cup\{ e\}) - \violations(X)
 = | N_{X}(u) \cap \overline{N}(v) | 
 + | N_{X}(v) \cap \overline{N}(u) |.
\]
It is now easy to see that for 
$X\subseteq Y\subseteq E$
and any $u\in V$ we have 
\[ 
| N_{X}(u) \cap W | \le | N_{Y}(u) \cap W |, 
\]
and thus, for $X\subseteq Y\subseteq E$
and any edge
$e=(u,v)\not\in Y$ it is
\[ 
\violations(X\cup\{ e\}) - \violations(X)
\le \violations(Y\cup\{ e\}) - \violations(Y),
\]
which proves the proposition.
\end{proof}

\begin{proposition}
	The function $\violations(X)$ is {\em monotone non-decreasing} supermodular with respect to
	the set of \strong-edges $X$.
\end{proposition}

\begin{proof}
Consider an \strong-edge sets $X$ and $Y$, such that $X\subseteq Y\subseteq E$. A number of violations, induced by set $Y$ can be expressed by sum of violations induced by each edge $(u,v)\in Y$. One half is needed as each violated triangle is considered twice, because it is caused by two \strong-edges.

\begin{equation*}
\begin{split}
\violations(Y) = & 
\frac{1}{2}\sum_{(u,v)\in Y}
{| N_{Y}(u) \cap \overline{N}(v) | 
	+ | N_{Y}(v) \cap \overline{N}(u) |}
\end{split}
\end{equation*}

Set of violated triangles induces by $Y$ consists of open triangles with two edges $e_1$ and $e_2$, such that $e_1\in X$ and $e_2\in X$ or $e_1\in Y\setminus X$ and $e_2\in Y\setminus X$; or $e_1\in X$ and $e_2\in Y\setminus X$:


\begin{equation*}
\begin{split}
\violations(Y) = & 
\frac{1}{2}\sum_{(u,v)\in X}
{| N_{X}(u) \cap \overline{N}(v) | 
	+ | N_{X}(v) \cap \overline{N}(u) |} + \\
&
\frac{1}{2}\sum_{(u,v)\in Y\setminus X}
{| N_{Y\setminus X}(u) \cap \overline{N}(v) | 
	+ | N_{Y\setminus X}(v) \cap \overline{N}(u) |} + \\
&
\sum_{(u,v)\in X}
{| N_{Y\setminus X}(u) \cap \overline{N}(v) | 
	+ | N_{Y\setminus X}(v) \cap \overline{N}(u) |}
\end{split}
\end{equation*}
Thus, the following inequality holds for any \strong-edge sets $X$ and $Y$, such that $X\subseteq Y\subseteq E$:
\[
\violations(Y) \geq \frac{1}{2}\sum_{(u,v)\in X}
{| N_{X}(u) \cap \overline{N}(v) | 
	+ | N_{X}(v) \cap \overline{N}(u) |} = \violations(X)
\]
Therefore, \violations($\cdot$) is non-decreasing monotone set function. 
\end{proof}

Let $X$ be a set of all \strong-edges in a connected graph $G$, denote set of all \weak-edges in $G$ by $A=E\setminus X$.
\begin{proposition}
A system $\matroid=(E,\independent)$ with set of independent sets \independent=\{$A\subseteq E$, such that $G(E\setminus A)$ is connected\} is a matroid.
\end{proposition}

\begin{proof}
\begin{enumerate}
\item
{Show that empty set is independent.
	
Let $A=\emptyset$, then $E\setminus A=E$ and $G(E)$ is connected. Thus $A\in \independent$.
}
\item
{
Hereditary property: every subset of an independent set is independent.
Show that if $A\in \independent$ and $B\subset A$, then $B\in \independent$.

If $A\in \independent$, then $G(E\setminus A)$ is connected. Since $B\subset A$, then $E\setminus A \subset E\setminus B$ and $G(E\setminus B)$ is connected as a supergraph of a connected graph. Thus $B\in \independent$.
}
\item
{
Augmentation property. Show that for any  $A\in \independent$ and $B\in \independent$ with $|B|<|A|$, there exists an element $e\in A$, such that $B\cup\{e\}\in \independent$ and  $|B\cup\{e\}|>|B|$.

First note that, since $A\in \independent$, then every edge $e=(u,v)\in A$ participates in at least one cycle $C\in (E\setminus A)\cup \{e\}$, which contains exactly one edge from $A$. Otherwise, $G(E\setminus A)$ does not contain a path from $u$ to $v$ and $G(E\setminus A)$ is disconnected. Let us refer to such cycles as \strong-cycles.

Case 1: there is an edge $e=(u,v)\in A\setminus B$, which participates in a \strong-cycle $C\in (E\setminus A)\cup \{e\}$ and $C\cap B=\emptyset$ (the cycle does not intersect $B$). That means that $C\in G(E\setminus B)$ and $\{e\}\in C$. Thus, $G((E\setminus B) \setminus\{e\})$ remains connected and $B\cup \{e\}\in \independent$.

Case 2: there is no edge $e\in A\setminus B$, which participates in a \strong-cycle with no edge form $B$. Thus, every \strong-cycle for any edge $e=(u,v)$ has the structure $C=(u,X_u,b_u,\dots,\allowbreak b_v,X_v,v,u)$, where $X_u$ and $X_v\subseteq E\setminus (A\cup B)$, $b_u$ - start node of the first visited edge in $B$, $b_v$ - end node of the last visited edge in $B$.

If $A\setminus B$ contains exactly one edge, then by assumption of the case in hand $B\setminus A$ contains at least one edge and requirement $|B|<|A|$ is violated.

If for some two edges $e_1=(u_1,v_1)$ and $e_2 = (u_2,v_2)\in A\setminus B$, there exist \strong-cycles, which share the same $b_v$ and $b_u$: $C_1=(u_1,X_{u_1},b_u,\dots,\allowbreak b_v,X_{v_1},v_1,u_1)$ and $C_2=(u_2,X_{u_2},b_u,\dots,\allowbreak b_v,X_{v_2},v_2,u_2)$, then there is a cycle $C$, constructed by the parts of these \strong-cycles, which belongs to $E\setminus B$ and contains $e_1$ and $e_2$: $C=(u_1,X_{u_1},b_u,X_{u_2},u_2,v_2,X_{v_2}, \allowbreak b_v,X_{v_1},v_1,u_1)\in (E\setminus(A\cup B)) \cup \{e_1\}\cup \{e_2\}$. Thus, $G((E\setminus B) \setminus\{e_1\})$ is connected and $B\cup \{e_1\}\in \independent$. 

If none of two edges in $A\setminus B$ have corresponding \strong-cycles with the same pair $(b_u,b_v)$, then $B\setminus A$ contains at least $|A|$ unique pairs of connected nodes $(b_u,b_v)$. Thus, $B\setminus A$ has at least $|A|$ edges. That contradicts with the property $|B|<|A|$. 

Consequently, there is always a cycle in $E\setminus B$ with at least one edge  $e\in A\setminus B$, and $B\cap \{e\}\in \independent$.
}
\end{enumerate}
\end{proof}

Intersection of Matroids: Consider a set of matroids over the same ground set $E$: $\matroid_1=(E,\independent_1),\matroid_2=(E,\independent_2), \dots, \matroid_k=(E,\independent_k)$. Intersection of matroids is $\matroid=(E,\independent)$ with $\independent=\{A\subseteq E, \text{ such that } A\in \independent_i \text{ for } 1\leq i\leq k\}$.

Define $\covered(A)$ to be the number of open triangles, which are preserved unviolated by set of \weak-edges $A$. Denote number of all open triangles in $G$ as $T$. Then $\covered(A) = T-\violations(X)$. A set function $\covered(A)$ is submodular non-decreasing function.

\begin{problem}
Given a graph $G=(V,E)$ 
and a set of teams 
$T_1,\ldots, T_k\subseteq V$.
The objective is to infer the type of edges of $E$ as \strong\ or \weak, 
so that all given teams are \strong-connected and the number
of non-violated triangles is maximized.
\label{problem:stcSifthed}
\end{problem}

Problem \ref{problem:stcSifthed} is a submodular maximization problem with intersection of matroids constraint: find a set of edges $A\subseteq E$ (edges with label \weak), such that $\covered(A)$ is maximized and $A \in \independent=\{A\subseteq E, \text{ such that } G_i(E\setminus A) \text{ is connected } \text{ for } 1\leq i\leq k\}$.

In as been shown that submodular maximization problem subjected to intersection of matroids can be solved greedily by Algorithm \ref{alg:greedySConnect} with $\frac{1}{k+1}$ approximation guarantee \cite{fisher1978analysis}. 

\begin{algorithm}
	\caption{Greedy for S-connectivity Problem}
	\label{alg:greedySConnect}
	%\begin{algorithmic}			
		{$A=\emptyset$, $V=E$}\;
		\While{$V\ne \emptyset$}{		
		{$e=\argmax_{e \in V}(\covered(A\cup\{e\})-\covered(A))$} 
		\tcc{the same as $e=\argmax(\violations(E\setminus A)-\violations(E\setminus A\setminus\{e\}))$}
		\If{$A\cup\{e\}\in \independent$}{
		%\Comment all teams are \strong-connected
		{$A = A\cup\{e\}$}
		}
		{$V = V\setminus\{e\}$}
		}
		\Return $A$\;
		\KwResult {Set of \weak-edges $A$}
	%\end{algorithmic}
\end{algorithm}
\fi

